A Graph-Transformational Approach for Proving the Correctness of Reductions between NP-Problems

The complexity class NP of decision problems that can be solved nondeterministically in polynomial time is of great theoretical and practical importance where the notion of polynomial-time reductions between NP-problems is a key concept for the study of NP. As many typical NP-problems are naturally described as graph problems, they and their reductions are obvious candidates to be investigated by graph-transformational means. In this paper, we propose such a graph-transformational approach for proving the correctness of reductions between NP-problems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{76}
\providecommand{\publicationstatus}{R. Heckel and C.M. Poskitt (Eds.): 13th International\\ Workshop on Graph Computation Models (GCM 2022)\\
EPTCS 374, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.374.7}{10.4204/EPTCS.374.7}}


==> tikz/proofprocfcommons.tex <==
\node(G){$G$};
\node(H)[below = 2 of G]{$H$};
\node(Gbar)[right = 2 of G]{$AS_0$};
\node(redG)[right = 2 of Gbar]{$\red(G)$};
\node(Hbar)[right = 2 of H]{$H_0$};

